MC-CoT: A Modular Collaborative CoT Framework for Zero-shot Medical-VQA with LLM and MLLM Integration

In recent advancements, multimodal large language models (MLLMs) have been fine-tuned on specific medical image datasets to address medical visual question answering (Med-VQA) tasks. However, this common approach of task-specific fine-tuning is costly and necessitates separate models for each downstream task, limiting the exploration of zero-shot capabilities. In this paper, we introduce MC-CoT, a modular cross-modal collaboration Chain-of-Thought (CoT) framework designed to enhance the zero-shot performance of MLLMs in Med-VQA by leveraging large language models (LLMs). MC-CoT improves reasoning and information extraction by integrating medical knowledge and task-specific guidance, where LLM provides various complex medical reasoning chains and MLLM provides various observations of medical images based on instructions of the LLM. Our experiments on datasets such as SLAKE, VQA-RAD, and PATH-VQA show that MC-CoT surpasses standalone MLLMs and various multimodality CoT frameworks in recall rate and accuracy. These findings highlight the importance of incorporating background information and detailed guidance in addressing complex zero-shot Med-VQA tasks.

==> Tables/change_module.tex <==
\begin{table*}
\centering
\begin{tabular}{l|cccccc|cc}
\toprule
\multicolumn{1}{l|}{}& \multicolumn{2}{c}{PATH-VQA} & \multicolumn{2}{c}{VQA-RAD} &\multicolumn{2}{c|}{SLAKE} &\multicolumn{2}{c}{Avg.}\\
& Recall & Acc.& Recall & Acc.& Recall & Acc.& Recall&Acc.\\
\midrule
MC-CoT(\emph{w/o rad}) &49.06 &35.41& 56.04 &31.75& \textbf{70.16}&52.14& 58.42& 39.77\\
MC-CoT(\emph{w/o pth}) &\textbf{49.93} &37.12& 56.30 &33.58&69.71 &52.51& 58.65&41.07 \\
MC-CoT(\emph{w/o ana}) &49.72&37.33&55.88 & 34.53 & 69.19& 52.87& 58.26& 41.58 \\
MC-CoT &49.90 &\textbf{45.10}&\textbf{57.06 } &\textbf{38.25}&69.82 &\textbf{54.88}&\textbf{58.93} & \textbf{46.08}\\ 
\bottomrule
\end{tabular}
\caption{The impact of the 3 modules on the effectiveness of the MC-CoT framework.
}
\label{tab:change-module}
\end{table*}
